Values That Are Explicitly Present in Fairy Tales: Comparing Samples from German, Italian and Portuguese Traditions

Looking at how social values are represented in fairy tales can give insights about the variations in communication of values across cultures. We study how values are communicated in fairy tales from Portugal, Italy and Germany using a technique called word embedding with a compass to quantify vocabulary differences and commonalities. We study how these three national traditions differ in their explicit references to values. To do this, we specify a list of value-charged tokens, consider their word stems and analyse the distance between these in a bespoke pre-trained Word2Vec model. We triangulate and critically discuss the validity of the resulting hypotheses emerging from this quantitative model. Our claim is that this is a reusable and reproducible method for the study of the values explicitly referenced in historical corpora. Finally, our preliminary findings hint at a shared cultural understanding and the expression of values such as Benevolence, Conformity, and Universalism across the studied cultures, suggesting the potential existence of a pan-European cultural memory.

==> tikz-header.tex <==
\usetikzlibrary{shapes, arrows.meta, calc, positioning, shadows}
% taken from manual
\makeatletter


\tikzset{
    rect/.style n args={4}{
        draw=none,
        rectangle,
        append after command={
            \pgfextra{%
                \pgfkeysgetvalue{/pgf/outer xsep}{\oxsep}
                \pgfkeysgetvalue{/pgf/outer ysep}{\oysep}
                \def\arg@one{#1}
                \def\arg@two{#2}
                \def\arg@three{#3}
                \def\arg@four{#4}
                \begin{pgfinterruptpath}
                    \ifx\\#1\\\else
                        \draw[draw,#1] ([xshift=-\oxsep,yshift=+\pgflinewidth]\tikzlastnode.south east) edge ([xshift=-\oxsep,yshift=0\ifx\arg@two\@empty-\pgflinewidth\fi]\tikzlastnode.north east);
                    \fi\ifx\\#2\\\else
                        \draw[draw,#2] ([xshift=-\pgflinewidth,yshift=-\oysep]\tikzlastnode.north east) edge ([xshift=0\ifx\arg@three\@empty+\pgflinewidth\fi,yshift=-\oysep]\tikzlastnode.north west);
                    \fi\ifx\\#3\\\else
                        \draw[draw,#3] ([xshift=\oxsep,yshift=0-\pgflinewidth]\tikzlastnode.north west) edge ([xshift=\oxsep,yshift=0\ifx\arg@four\@empty+\pgflinewidth\fi]\tikzlastnode.south west);
                    \fi\ifx\\#4\\\else
                        \draw[draw,#4] ([xshift=0+\pgflinewidth,yshift=\oysep]\tikzlastnode.south west) edge ([xshift=0\ifx\arg@one\@empty-\pgflinewidth\fi,yshift=\oysep]\tikzlastnode.south east);
                    \fi
                \end{pgfinterruptpath}
            }
        }
    },
    rect'/.style n args={4}{
        rectangle,
        append after command={
            \pgfextra{%
                \pgfkeysgetvalue{/pgf/outer xsep}{\oxsep}
                \pgfkeysgetvalue{/pgf/outer ysep}{\oysep}
                \begin{pgfinterruptpath}
                    \ifx\\#1\\\else
                        \draw[draw,#1] ([xshift=-\oxsep,yshift=0]\tikzlastnode.south east) edge ([xshift=-\oxsep,yshift=0]\tikzlastnode.north east);
                    \fi\ifx\\#2\\\else
                        \draw[draw,#2] ([xshift=-\pgflinewidth,yshift=-\oysep]\tikzlastnode.north east) edge ([xshift=0+\pgflinewidth,yshift=-\oysep]\tikzlastnode.north west);
                    \fi\ifx\\#3\\\else
                        \draw[draw,#3] ([xshift=\oxsep,yshift=0-\pgflinewidth]\tikzlastnode.north west) edge ([xshift=\oxsep,yshift=0+\pgflinewidth]\tikzlastnode.south west);
                    \fi\ifx\\#4\\\else
                        \draw[draw,#4] ([xshift=0+\pgflinewidth,yshift=\oysep]\tikzlastnode.south west) edge ([xshift=0-\pgflinewidth,yshift=\oysep]\tikzlastnode.south east);
                    \fi
                \end{pgfinterruptpath}
            }
        }
    },
    dontshortenme/.style={
        shorten >=0pt,
        shorten <=0pt
    },
    rect''/.style n args={4}{
        draw=none,
        rectangle,
        append after command={
            \pgfextra{%
                \pgfkeysgetvalue{/pgf/outer xsep}{\oxsep}
                \pgfkeysgetvalue{/pgf/outer ysep}{\oysep}
                \def\my@path{\path[shorten >=\pgflinewidth,shorten <=\pgflinewidth] ([xshift=-\oxsep]\tikzlastnode.south east) edge}
                \def\arg@{#1}
                \ifx\arg@\@empty
                    \def\arg@{draw=none}
                \fi
                \eappto\my@path{[\arg@] }
                \appto\my@path{ ([xshift=-\oxsep]\tikzlastnode.north east)
                                          ([yshift=-\oysep]\tikzlastnode.north east) edge }
                \def\arg@{#2}
                \ifx\arg@\@empty
                    \def\arg@{draw=none}
                \fi
                \eappto\my@path{[\arg@] }
                \appto\my@path{ ([yshift=-\oysep]\tikzlastnode.north west)
                                          ([xshift=\oxsep] \tikzlastnode.north west) edge }
                \def\arg@{#3}
                \ifx\arg@\@empty
                    \def\arg@{draw=none}
                \fi
                \eappto\my@path{[\arg@] }
                \appto\my@path{ ([xshift=\oxsep]\tikzlastnode.south west)
                                          ([yshift=\oysep] \tikzlastnode.south west) edge }
                \def\arg@{#4}
                \ifx\arg@\@empty
                    \def\arg@{draw=none}
                \fi
                \eappto\my@path{[\arg@] }
                \appto\my@path{ ([yshift=\oysep]\tikzlastnode.south east);}
                \begin{pgfinterruptpath}
                    \my@path
                \end{pgfinterruptpath}
            }
        }
    }
}

\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ‘‘flipped page’’
\pgf@xc=\pgf@xb \advance\pgf@xc by-10pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-10pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother

\tikzstyle{doc}=[%
draw,
thick,
align=center,
color=black,
shape=document,
minimum width=2,
minimum height=2.8,
shape=document,
inner sep=2ex,
]

